Symbolic Timed Observational Equivalence

Intruders can infer properties of a system by measuring the time it takes for the system to respond to some request of a given protocol, that is, by exploiting time side channels. These properties may help intruders distinguish whether a system is a honeypot or concrete system helping him avoid defense mechanisms, or track a user among others violating his privacy. Observational equivalence is the technical machinery used for verifying whether two systems are distinguishable. Moreover, efficient symbolic methods have been developed for automating the check of observational equivalence of systems. This paper introduces a novel definition of timed observational equivalence which also distinguishes systems according to their time side channels. Moreover, as our definition uses symbolic time constraints, it can be automated by using SMT-solvers.

==> autoverif.tex <==
%!TEX root = obseq.tex
\section{Automating Verification}
\label{autoverif}
We detail in this section our Maude formalization which allows us
to automatically check whether two initial configurations are timed equivalent. 

To make analysis feasible we use a symbolic semantics for intruder
interactions as well as for time constraints.  To further facilitate
implementation of analysis, the semantics
records events making traces/bundles explicit rather than implicit.
Thus a \emph{Maude configuration} has the form 

\begin{verbatim}
    pc ! tSym ! ds ! b ! exe
\end{verbatim}
where  
\begin{itemize}
\item  
\texttt{pc} is the player configuration consisting of honest players \texttt{[h(i),j | evtl | keys]} each with their associated intruder \texttt{[I(i),j| msgs | buff ]}. Here \texttt{evtl} is the timed protocol that the player follows (coding a role $\pl$); \texttt{i,j} are natural numbers used for player identification and ensuring nonce freshness; \texttt{keys} are the keys possessed by the player; \texttt{msgs} are the (symbolic) messages that have been learned by the intruder, \ie, his current knowledge; \texttt{buff} contains messages that have been shared by other intruders and that have not yet been learned by the intruder because they still did not arrive the intruder.
\item  
\texttt{ds} is the set of constraints on intruder generated symbols
\item  
\texttt{tSym} is the symbolic current time
\item  
\texttt{b} the symbolic time constraints, includes network topology
    $r_0 \le  \key{td}(i,j) \le  r_1$
\item  
\texttt{exe} a sequence of message transmission events 
\texttt{o(msg,sndr,rcvr,ts)}.  Each \texttt{ds} instance  of \texttt{exe} (see definition \ref{ds-model} below) corresponds directly
 to a timestamped bundle.
\end{itemize}

Messages delivered to honest players by intruders are symbols
constrained to be derivable from the intruders current knowledge. The
messages are also constrained to be receivable, formalizing the
implicit meaning of message patterns. For example, a pattern
\texttt{-(enc(x,y))} implies the receiver has the decryption key.

By using symbolic terms, a single Maude configuration can represent a number of timed bundles. For example, consider the following Maude configuration with one player \texttt{H(0)} and his associated intruder \texttt{I(0)} 

\begin{verbatim}
[h(0),3 | eif vs(0, 1) :=: e(vs(0, 0), KM) 
           # tt(1) := tt(5) + tMac 
           ethen ... | sk(pv("A"))]
[I(0),1 | sk(p("I:0")) n(0,0) | m-old
 e(n(0,1000),KE) e(e(n(0,1000),KE),KM)] ! tt(5) 
! dc(vs(0, 0), z(n(0, 0) m-old)) 
  dc(vs(0, 1), z(n(0, 0) m-old)) 
! tt(5) >= 0 and tMac >= 1.0 and tEnc >= 2.0 
  and tt(6) >= tt(5)
! o(n(0,0),(h(0),1),(I(0),1),tt(5)) ;
  o({vs(0,0),vs(0,1)},(I(0),0),(h(0),2),tt(6))
\end{verbatim}

The honest player is executing the passport protocol described in Example~\ref{ex:passport}. Part of the protocol is omitted, represented by the ellipses \texttt{...}.  \texttt{m-old} stands for the messages \texttt{e(n(0,-1),KE) e(e(n(0,-1),KE)} which are  messages, corresponding to $\m_{enc}^{old}, \m_{mac}^{old}$, learned by the intruder in a previous protocol session. 

The protocol has already started as can be verified by the two message transmission events in the \texttt{exe} component: the honest player has sent the nonce \texttt{n(0,0)} which was intercepted by the intruder \texttt{I(0)}. The intruder then sent a pair of symbols \texttt{{vs(0,0),vs(0,1)}} to the honest player. These symbols are constrained as specified by the \texttt{ds} component. In particular, they can be any message constructed using the term learned by the intruder until them, namely: \texttt{sk(p("I:0")) n(0, 0) m-old}.

This Maude configuration corresponds, therefore, to all timed bundles where the player sends a nonce and the intruder responds with any message constructed using \texttt{sk(p("I:0")) n(0, 0) m-old}. 

% The following relation defines all the possible messages that can be assigned to a symbol:
% \begin{itemize}
%   \item $\texttt{vs},\texttt{ds} \vdash \texttt{m}$ if $\texttt{m} \in \texttt{ds}$;
%   \item $\texttt{vs},\texttt{ds} \vdash \texttt{m}$ if $\texttt{vs'} \in \texttt{ds}$ and $\texttt{vs'},\texttt{ds} \vdash \texttt{m}$;

%   \item $\texttt{vs},\texttt{ds} \vdash \{\texttt{m}_1,\ldots,\texttt{m}_n\}$ if for all $1 \leq i \leq n$. $\texttt{vs},\texttt{ds} \vdash \texttt{m}_i$;

% \end{itemize}


% \red{VN:We may need a definition here}
% We write $\texttt{m},\texttt{ds} \vdash \m$ whenever the message $\m$, \ie, containing no symbols, can be generated from \texttt{m} by instantiating symbols satisfying \texttt{ds} to messages. 

The executable semantics of for timed protocols is specified by the rewrite rules in Figure~\ref{fig:rewrite-rules}. The whole specification can be found in~\cite{maude-timed}. We explain these rewrite rules in detail:\footnote{In order for improving clarity the rules here differ from the rules~\cite{maude-timed}, but are essentially the same.}
\begin{itemize}
  \item Rule \texttt{snd}: If a honest player \texttt{h(n)} is sending a message \texttt{t}, then this message is learned immediately by the intruder \texttt{I(n)} associated to \texttt{h(n)}. Moreover, it is added to the buffer of the remaining intruders, \texttt{I(m)}, to be learned after it arrives the intruder, at $\texttt{T} + \key{td}(n,m)$. This is specified by the function \texttt{bufAdd(n,t,T,pc)};

  \item Rule \texttt{asnd}: Its behavior is similar to the rule \texttt{snd}, but we replace all the occurrences of the time variable \texttt{T1} being assigned by the expression \texttt{TR1} replacing the keyword \texttt{cur} by the global time \texttt{T};

  \item Rule \texttt{tsnd}: Its behavior is similar to the rule  \texttt{snd}, but it only succeeds if the condition \texttt{b'} associated to the timed input \texttt{t} together with the accumulated time constraints \texttt{b} is satisfiable. To check this, we create a fresh global time \texttt{tt(s m)} which is greater or equal than the global time \texttt{tt(m)}. Then we replace the keyword \texttt{cur} in \texttt{b'} by \texttt{tt(s m)} and check whether the resulting formula \texttt{b2} is satisfiable. The rule can fire only if it is satisfiable. We use the SMT solver CVC4 to check whether the formula \texttt{b2} is satisfiable. This is specified by the command \texttt{(metaCheck(['EXE],toVarsB(b2)))} which returns true if it is satisfiable and false otherwise;

  \item Rule \texttt{newN}: This rule creates a new nonce \texttt{n(i,j)}. The indexes \texttt{i,j} are used to ensure its freshness. We then replace all occurrences of the variable \texttt{nv:nonceVar} in the remaining protocol specification \texttt{evtl} by \texttt{n(i,j)}. This is done by using the substitution \texttt{sb}.

  \item Rule \texttt{rcv}: This rule specifies the when a honest player \texttt{h(n)} is expecting to receive a message \texttt{t}. Under the timed intruder model, this message is sent by his associated intruder \texttt{I(n)}. However, instead of sending a concrete message, we use symbolic terms which reduces search space. 
Given the term \texttt{t}, the set of current symbol constraints
\texttt{ds}, and the intruder’s current knowledge \texttt{ts}, we compute
(\texttt{sGen}) the possible messages the intruder can construct that can
be received by the honest player \texttt{h(n)}. This set is represented
symbolically as \texttt{\{sb, css1\}} where \texttt{sb} maps variables of
\texttt{t} to new symbols, and \texttt{css1} is a set of pairs
\texttt{\{ssb1, ds1\}} where \texttt{ssb1} maps some symbols to terms (a
partial solution to the constraints) and \texttt{ds0} extends ds1 with
additional constraints needed to match the term \texttt{t}.
(\texttt{css1} is written as \texttt{\{ssb, ds0\}, css} in the rule
condition to ensure the set is not empty, and to pick one to use).
\texttt{sGen} uses both matching and unification to find solutions to the
generation problem.

  \item Rule \texttt{buff}: This rule specifies when an intruder, \texttt{iid}, learns a message \texttt{t} that was sent by another intruder and should reach \texttt{iid} at time \texttt{TR}. For this we create a fresh time symbol \texttt{t(s j)} which is greater than \texttt{t(j)} and is greater than the time \texttt{TR} when the message \texttt{t} is supposed to reach the intruder \texttt{iid}. This is specified by the new timed constraint \texttt{b'};

  \item Remaining Rules: We omitted for space reasons the rules specifying the semantics of timed receives, \texttt{(-t) \# b} and \texttt{(-t) \# T1 := TR1}, and conditionals. Their semantics are as expected. The receive rules additionally add time constraints, while the conditional checks whether the condition is true or not. The complete specification can be found in \cite{maude-timed}.
\end{itemize}

\begin{figure*}[t]
  \begin{verbatim}
rl[snd]: 
[h(n), j | +(t), evtl | ks] pc ! T ! ds ! b ! exe 
=>  
[h(n), s j | evtl | ks] bufAdd(n,t,T,pc) ! T ! ds ! b ! exe ; o(t,(h(n),j),(I(n),j),T)

crl[asnd]:
[h(n), j | +(t # T1 := TR1), evtl | ks] pc ! T ! ds ! b ! exe 
=>
[h(n), s j | tsubl(T1,TR2,evtl) | ks] bufAdd(n,t,T,pc) ! T ! ds ! b !
      exe ; o(t,(h(n),j),(I(n),j),T)
if TR2 := tsubr(cur,T,TR1) . 

crl[tsnd]:
[h(n), j | +(t # b'), evtl | ks] pc ! tt(m) ! ds ! b ! exe 
 =>
[h(n), s j | evtl | ks] bufAdd(n,t,tt(s m),pc) ! tt(s m) ! ds ! b2 ! 
       exe ; o(t,(h(n),j),(I(n),j),tt(s m))
if b1 := (tt(s m) >= 0/1) and (tt(s m) >= tt(m) and (b))
/\ b2 := tsubb(cur,tt(s m),b') and (b1) 
/\ (metaCheck(['EXE],toVarsB(b2))) .  

crl[newN]:
[h(i), j | new(nv:nonceVar), evtl | ks] pc ! T ! ds ! b ! exe 
=>
[h(i), s j | sb[[evtl]] | ks] pc ! T ! ds ! b ! exe 
if sb := nv:nonceVar := n(i,j) .

crl[rcv]:
[h(n), j | -(t), evtl | ks] [I(n),i | ts | tts ] pc ! T ! ds ! b ! exe
=>
[h(n), s j | ssb[[sb[[evtl]]]] | 
addKeys(t,sb0,ssb[[[ks]]])] [I(n), s i | ssb[[[ts]]] | ssb[[[tts]]] ] ssbPC(ssb,pc) ! T
! ds0 ! b ! ssbExe(ssb,exe) ;  o(ssb[sb0[t]],(I(n),i),(h(n),j),T) 
if {sb,{ssb,ds0} css} := sGen(n,i,t,ts,ds) 
/\ sb0 := ssbRng(ssb,sb,mtS)
/\ receivable(t,sb0,ks) .  

crl[buff]:
[iid, i | ts | (t @ TR1) tts ] pc ! (tt(j)) ! ds !  b ! exe  
=>
pc ! (tt(s j)) ! ds ! b' ! exe
b' := (tt(s j) >= 0/1) and (tt(s j) >= tt(j) and (tt(s j) >= TR1 and b)) .
\end{verbatim}
\caption{Rewrite rules specifying the executable semantics for timed bundles. The rules for timed receive commands and conditionals are omitted. \texttt{pc} is a variable for a set of honest players and intruders.}
\label{fig:rewrite-rules}
\end{figure*}

\smallskip

In order to connect symbolic executions to concrete ones we need to
define the notion of model for the intruder symbol constraints 
\texttt{ds}.
\begin{definition}\label{ds-model}
A \emph{model} $M$ of a set of intruder symbol constraints \texttt{ds}
is a (sort preserving) mapping from the symbols in \texttt{ds}
(domain and range) to ground terms such that for each 
\texttt{s} in the domain of $M$ that is constrained by \texttt{ds}
(\texttt{ds} contains \texttt{dc(s,z(ts-1)...z(ts-k))}),
$M(\texttt{s})$ is derivable from each set $M(\texttt{ts-i})$ 
$1 \le i \le k$.
In this case we write $M \vdash \texttt{ds}$ 
\end{definition}

Note that the definition is well-defined due to the fact that
\texttt{ds} is required to be non-cyclic.
Given a Maude configuration reachable from a Maude initial configuration,
the execution component of that
Maude configuration represents the concrete executions obtained
by applying substitutions that model the symbol constraint
component.

The following soundness and completeness theorem can be proved by 
extending the corresponding result (to appear elsewhere) 
for untimed protocols as the
treatment of time constraints is independent from the symbol
constraints.  

\begin{theorem}
\label{the:sound-complete}
   Let $I = \tup{\Hscr,\Iscr,\key{td}}$ be an initial configuration. Let \texttt{I} be the initial Maude configuration corresponding to $I$. There is a one to one correspondence between the timed bundles $\Sscr(I)$ and the concrete executions of Maude configurations reachable using the rules in Figure~\ref{fig:rewrite-rules}.
\end{theorem}



% \begin{definition}
% Let \texttt{C = pc ! tSym ! ds ! b ! exe} be a configuration. The set of instances of \texttt{C} is the set of configurations:
% \[
% \left\{\begin{array}{lcl}
% \texttt{C}\sigma & \mid & \textrm{for all ground substitutions } \sigma\\
% && \textrm{mapping term symbols \texttt{vs} to messages \m}\\
% && \textrm{such that $\texttt{vs},\texttt{ds} \vdash \m$.}   
% \end{array}\right\}  
% \]
% \end{definition}

% For a configuration  the set of observations instance of \texttt{C} is the set:



% as the tuple \texttt{b ! ds ! exe-obs}, where \texttt{exe-obs} is \texttt{exe} to messages that are sent by honest players to intruders (following Definition~\ref{def:message-observation}). Thus the observations of the configuration shown above is simply \texttt{o(n(0,0),(h(0),1),(I(0),1),tt(5))}.  

% \begin{definition}
%   A set of observations, $\Oscr(\Cscr), \TC(\Cscr,\key{td})$, of a timed bundle $\Cscr$ is contained in the set of observations \texttt{b ! ds ! exe-obs} of a configuration \texttt{C} if for all models $M \vDash \TC(\Cscr,\key{td})$ there is a model $M_1 \vDash \texttt{b}$ such that for each observation $\tup{m,\p,I_\p,\tv}$, there is an observation in \texttt{exe-obs} with message $\texttt{m}$ sent by $\p$ and received by $\p_I$ at time \texttt{tt} such that $\texttt{m},\texttt{ds} \vdash \m$ and $M[\tv] = M_1[\texttt{tt}]$.  
% \end{definition}

% The following theorem is proved by induction on the size of derivations. 

% \begin{theorem}[Same Observations]
%   Let $I = \tup{\Hscr,\Iscr,\key{td}}$ be an initial configuration. Let \texttt{I} be the Maude initial configuration specifying $I$. The following properties are valid:
% \begin{itemize}
%   \item \textbf{Soundness} For any 


%    For any timed bundle $\Cscr \in \Sscr(I)$, there is a reduction 
%   \texttt{I} $\rightarrow^*$ \texttt{C} such that the observations of $\Cscr$ are contained in the observations of \texttt{C};

%   \item \textbf{Completeness} For any timed bundle $\Cscr \in \Sscr(I)$, there is a reduction 
%   \texttt{I} $\rightarrow^*$ \texttt{C} such that the observations of $\Cscr$ are contained in the observations of \texttt{C};

% \end{itemize}
% \end{theorem}


% \red{Do we have some theorem here?}

\subsection{Automating the Proof of Timed Equivalence}

We first show how one can prove whether two  Maude configurations are equivalent in the sense that for all timed bundles reprsented by $\texttt{C1}$ there is an equivalent timed bundle represented $\texttt{C2}$. We then proceed to show how two initial Maude configurations are equivalent.

\paragraph{Maude Configuration Equivalence:}
Consider two Maude configurations:
\[
\begin{array}{l}
\texttt{C1} = \texttt{pc1 ! tSym1 ! ds1 ! b1 ! exe1} \\[2pt]
\texttt{C2} = \texttt{pc2 ! tSym2 ! ds2 ! b2 ! exe2}   
\end{array}
\] 
We determine whether they are equivalent in the sense that for all timed bundles reprsented by  $\texttt{C1}$ there is an equivalent timed bundle represented $\texttt{C2}$.  Assume without loss of generality that \texttt{C1} and \texttt{C2} have disjoint term symbols and time variables. 

Let $\texttt{exe1}$ and \texttt{exe2} be the lists:
\[
\begin{array}{l}
  \texttt{exe1} = o(\texttt{m}_1,\texttt{snd}_1,\texttt{rcv}_1,\texttt{ts}_1),\ldots,o(\texttt{m}_n,\texttt{snd}_n,\texttt{rcv}_n,\texttt{ts}_n)] \\  
  \texttt{exe2} = o(\texttt{m}_1',\texttt{snd}_1',\texttt{rcv}_1',\texttt{ts}_1'),\ldots,o(\texttt{m}_n',\texttt{snd}_n',\texttt{rcv}_n',\texttt{ts}_n')] 
\end{array}
\]
Notice that if the executions have different sizes, then the Maude configurations are not equivalent. We proceed by checking whether the bijection 
\[
o(\texttt{m}_i,\texttt{snd}_i,\texttt{rcv}_i,\texttt{ts}_i) \leftrightarrow o(\texttt{m}_i',\texttt{snd}_i',\texttt{rcv}_i',\texttt{ts}_i')   
\]
for $1 \leq i \leq n$ is a witness for the timed equivalence of the timed bundles represented by \texttt{C1} and \texttt{C2}. This already means that the observations have the same senders and receivers, that is, $\texttt{snd}_i = \texttt{snd}_i'$ and $\texttt{rcv}_i = \texttt{rcv}_i'$, for all $1 \leq i \leq n$.

However, we face the following two main challenges in automating this verification:
\begin{enumerate}
  \item \textbf{Term Symbols:} The terms $\texttt{m}_i$ and $\texttt{m}_i'$ for all $1 \leq i \leq n$ may contain symbols. So simple equality will not work. We need to check whether the following formula $F$ is true
  \[
\begin{array}{l}
  \forall M_1. (M_1 \vdash \texttt{ds1} \Rightarrow \\
 \quad  \exists M_2. M_2 \vdash \texttt{ds2} \land \forall 1 \leq i\leq n. M_1[\m_i] \sim M_2[\m_i'] 
  )  
\end{array}
\]
and its converse.

 We can use our constraint solver to check whether $F$ is true. In particular, we check whether $\neg F$ is false, that is:
 \[
\begin{array}{l}
  \exists M_1. (M_1 \vdash \texttt{ds1} \land \\
 \quad \neg \exists M_2. M_2 \vdash \texttt{ds2} \land \forall 1 \leq i\leq n. M_1[\m_i] \sim M_2[\m_i'] 
  )  
\end{array}
\]
is false. This means that if we find models $M_1,M_2$, that unifies the messages, then $\neg F$ is false and consequently $F$ is true. Thus, we simply run our constraint solver (\texttt{sGen}) to check whether $\{\texttt{m}_1,\ldots,\texttt{m}_n\}$ is unifiable modulo encryption with $\{\texttt{m}_1',\ldots,\texttt{m}_n'\}$ provided $\texttt{ds1}$ and $\texttt{ds2}$. If there is a solution, then $F$ is true.

\item \textbf{Time Variables:} The second challenge is the quantification over all time models in the definition of time equivalence of timed bundles. In particular, we need to check the following formula $G$ is true:
\[
\begin{array}{l}
  \forall M_1. (M_1 \vDash \texttt{b1} \Rightarrow\\ 
\quad \exists M_2. (M_2 \vDash \texttt{b2} \land \forall 1 \leq i \leq n. M_1[\texttt{tsi}] = M_2[\texttt{tsi'}]))  
\end{array}
\]
and its converse. We proceed by checking whether its negation $\neg G$:
\[
\begin{array}{l}
  \exists M_1. (M_1 \vDash \texttt{b1} \land~\\ 
\quad \neg \exists M_2. (M_2 \vDash \texttt{b2} \land \forall 1 \leq i \leq n. M_1[\texttt{tsi}] = M_2[\texttt{tsi'}]))  
\end{array}
\]
is false. Thus if we are able to show that this formula is satisfiable, then we show that $\neg G$ is not false and thus $G$ is true. We can use an SMT solver to the check of whether $\neg G$ is satisfiable. In particular, we ask the SMT-solver to check whether the following formula is satisfiable: 
\[
  \texttt{b1} \land \neg (\texttt{b2} \land (\texttt{ts1} = \texttt{ts1'} \land \cdots \land \texttt{tsn} = \texttt{tsn'}))
\]
is satisfiable. Assume it is satisfiable with a model $M$. Recall that the time variables of \texttt{b1} and \texttt{b2} are disjoint. This means that there is a model of \texttt{b1}, namely $M$ restricted to the time variables in \texttt{b1}. Moreover, the formula $\exists M_2. (M_2 \vDash \texttt{b2} \land \forall 1 \leq i \leq n. M_1[\texttt{tsi}] = M_2[\texttt{tsi'}]$ is false. Thus, $\neg G$ is satisfiable and $G$ is true.
\end{enumerate}

\smallskip

If the two conditions (same terms and same times) are satisfied, then the Maude configurations \texttt{C1} and \texttt{C2} are equivalent, \ie, for each the timed bundles represented by \texttt{C1} there is an equivalent timed bundle represented by \texttt{C2} and the converse is true.

\paragraph{Initial Maude Configuration Equivalence}
We now use the machinery described above to show whether two initial Maude configurations \texttt{I1} and \texttt{I2} are equivalent. We first collect all the Maude configurations reachable from \texttt{I1} and \texttt{I2} that cannot be rewritten by the rules in Figure~\ref{fig:rewrite-rules}:
\[
  \begin{array}{c}
    \Rscr(\texttt{I1}) = \{\texttt{C1}, \ldots, \texttt{Cn}\} \quad \textrm{and} \quad
    \Rscr(\texttt{I2}) = \{\texttt{C1}', \ldots, \texttt{Cm}'\}
  \end{array}
\]
We then proceed as follows: For each $\texttt{C} \in \Rscr(\texttt{I1})$ (and conversely), we search for an equivalent Maude configuration $\texttt{C'} \in \Rscr(\texttt{I2})$ using the method described above.

% The following theorem is proved by using the reasoning above and Theorem~\ref{the:sound-complete}.

\begin{lemma}
  Two initial configurations $I_1 = \tup{\Hscr_1, \Iscr_1, \key{td}}$ and $I_2 = \tup{\Hscr_2, \Iscr_2, \key{td}}$ are timed equivalent if and only if their corresponding initial Maude configuration $\texttt{I1}$ and $\texttt{I2}$ are equivalent.
\end{lemma}

The following theorem establishes the decidability of the timed equivalence problem. This result  depends on the types of term contraints problems involved, \eg, assumptions on the encryption used, and time constraints problems involved, \eg, which theories used. 

\begin{theorem}
Assuming decidable term constraint and time constraint problems, the problem of checking whether two initial configurations $I_1 = \tup{\Hscr_1, \Iscr_1, \key{td}}$ and $I_2 = \tup{\Hscr_2, \Iscr_2, \key{td}}$ are timed equivalent is decidable.
\end{theorem}

The examples shown here all use decidable term and time contraints problems.


==> lang.tex <==
%!TEX root = obseq.tex
\section{Timed Protocol Specification Language}\label{lang}

This section reviews the timed protocol specification language introduced previously~\cite{nigam16esorics}.
\subsection{Syntax}

We start first by specifying the syntax of our protocol specification language with symbolic time variables and symbolic time constraints. We exemplify the specification of protocols using our language. Then, we formalize the operational semantics of our language by extending Strand Spaces~\cite{thayer99jcs} to include time variables.

\paragraph{Message Expressions}
We assume a message signature $\Sigma$ of constants, and function symbols. 
Constants include nonces, symmetric keys and player names.
The set of messages is constructed as usual using constants,  variables 
and at least the following function symbols:
\[
\begin{array}{l@{\qquad}p{5cm}}
  \sk(\p) & \textrm{Denoting the secret key of the player $\p$;}\\
  \pk(\p) & \textrm{Denoting the public key of the player $\p$;}\\
  \enc(\m,\k) & \textrm{Encryption function denoting the encryption of $m$ using key $k$;}\\
  \lst{\m_1,\m_2,\ldots,\m_n} & \textrm{Tuple function denoting a list of messages $\m_1,\m_2,\ldots,\m_n$;}\\
\end{array}  
\]
where $\c_1, \c_2, \ldots$ range over constants, 
$\n_1,\ldots,\n_n$ range over nonces,
$\k_1,\k_2,\ldots$ range over symmetric keys, 
$\p_1, \p_2 \ldots$ range over player names,
$\v_1,\v_2, \ldots$ range over variables, and
$\m_1,\m_2,\ldots$ range over messages.
For example, the message $\enc(\lst{\v_1, \enc(\c,\k)},\pk(\p))$ denotes the encryption using the public key of \p of the pair of messages $\v_1$ (not instantiated) and $\enc(\c,\k)$. We define $ (\pk(\p))^{-1} = \sk(\p)$ and $\k^{-1} = k$ if $\k$ is a symmetric key. We also write interchangeably the singleton tuple $\{\m\}$ and $\m$.

For a given scenario with some protocol session instances, we are going to distinguish the players that are participating in the protocol sessions, \eg, honest participants, which we call \emph{protocol participants} 
(briefly \emph{participants}), from the \emph{Timed Intruders} which are not participating explicitly in the protocol sessions in the given scenario, but are simply manipulating messages and possibly interacting with the participants. 
The symbols $\p_1, \p_2 \ldots$ will range over participant names
while  $\ti_1, \ti_2, \ldots$ will range over the names of such Timed Intruders. 

\paragraph{Time Expressions}
We also assume a time signature $\Xi$ which is disjoint to the message alphabet $\Sigma$. It contains:
\[
\begin{array}{l@{\quad}p{4cm}}
  \r_1,\r_2,\ldots & \textrm{A set of numbers;}\\
  \tv_1,\tv_2,\ldots,& \textrm{A set of time variables including the special variable $\cur$};\\
  +,-,\times,/, \floor,\ceiling, \ldots & \textrm{A set of arithmetic symbols and other function symbols.}
\end{array}  
\]
\emph{Time Expressions} are constructed inductively by applying arithmetic symbols to time expressions. For example $\ceiling((2 + \tv + \cur )/ 10)$ is a Time Expression. The symbols $\tr_1,\tr_2, \ldots$ range over Time Expressions.
We do not constrain the set of numbers and function symbols in $\Xi$. However, in practice, we allow only the symbols supported by the SMT solver used. All examples in this paper will contain SMT supported symbols (or equivalent). Finally, the time variable $\cur$ will be a keyword in our protocol specification language denoting the current global time.

\begin{definition}[Symbolic Time Constraints] Let $\Xi$ be a time signature.
The set of symbolic time constraints is constructed inductively using time expressions as follows: 
Let  
 $\tr_1,\tr_2$ be time expressions, then 
\[
\begin{array}{l}
  % \textrm{\textbullet~assignment:}~ \tv := \tr \\ 
  % \textrm{\textbullet~comparison:}~
  \tr_1 = \tr_2, \qquad \tr_1 \geq \tr_2 \qquad \tr_1 > \tr_2,\\\tr_1 < \tr_2, \quad \textrm{and} \quad \tr_1 \leq \tr_2
\end{array}
  % \textrm{\textbullet~assignment:}~ \tv := \tr \qquad \textrm{\textbullet~comparison:}~  \tr_1 \star \tr_2
\]
are Symbolic Time Constraints.
\end{definition}
For example, $\cur + 10 < \floor(\tv - 5)$ is a Time Constraint. 
The symbols $\tc_1, \tc_2, \ldots$ will range over Time Constraints.

Finally, we let $\b_1, \b_2, \ldots$, range over 
boolean expressions. We also allow for checking whether two messages $\m_1$ and $\m_2$ can be matched, \eg, $\lst{\v_1,\v_2} :=: \lst{\p_1, \k_1}$ evaluates to true as they can be matched by the substitution $\{\v_1 \mapsto \p_1,\v_2 \mapsto \k_1\}$. 

\begin{definition} [Timed Protocols]
The set of Timed Protocols, $\PL$, is composed of Timed Protocol Roles, $\pl$, which are constructed by using commands as specified by the following grammar, where $\b$ is a boolean expression:
\[
  \begin{array}{l@{\qquad}l}
     \mathsf{nil} & \textrm{Empty Protocol}\\
     \mid (\new~ \v), \mathsf{pl} & \textrm{Fresh Constant}\\
     \mid (+ \m), \mathsf{pl} & \textrm{Message Output}\\
     \mid (+ \m ~\#~ \tc), \mathsf{pl} &  \textrm{Timed Message Output}\\
     \mid (- \m), \mathsf{pl} & \textrm{Message Input}\\
     \mid (- \m ~\#~ \tc), \mathsf{pl} & \textrm{Timed Message Input}\\
     \mid (\myif{\b}{\mathsf{pl}_1}{\mathsf{pl}_2}) & \textrm{Conditional}\\
     \mid (\myif{\b~\#~\tc}{\mathsf{pl}_1}{\mathsf{pl}_2}) & \textrm{Timed Conditional}
  \end{array}
\]
\end{definition}

To identify a particular command in a Timed Protocol Role we use a string of the form $i_1.i_2.i_3.\ldots.i_n$, called position and denoted by $\bar{i}$, where each $i_j \in \{1,2\}$ to specify a path in the control flow of the Timed Protocol. For example, $1.1.1.1.2$ in Example~\ref{ex:passport} below leads to $(+ error ~\#~ \cur = \tv_1)$. We denote by $\mathcal{PS}(\pl)$ the set of strings representing the paths in the Timed Protocol Role $\pl$.

We explain some examples intuitively before we formalize the semantics of our language in the following section. We will elide $\mathsf{nil}$ whenever it is clear from the context.

\begin{example}
\label{ex:distance-bounding}
  The following role specifies the verifier of a (very simple) distance bounding protocol~\cite{brands93eurocrypt}:
  \[
  \begin{array}{l}
   (\new~\v),(+ \v~\#~\tv = \cur), (- \v~\#~\cur \leq \tv + 4) 
  \end{array}    
  \]
  It creates a fresh constant and sends it to the prover, 
  remembering the current global time by assigning it to the time variable $\tv$. Finally, when it receives the response $\v$ it checks whether the current time is less than $\tv + 4$.
\end{example}

\begin{example}[Passport]
\label{ex:passport}
Timed conditionals can be used to specify the duration of operations, such as checking whether some message is of a given form. In practice, the duration of these operations can be measured empirically to obtain a finer analysis of the protocol~\cite{chothia10fc}.

For example, consider the following protocol role: 
\[
\begin{array}{l}
  (\new~\v),(+ \v),(- \{\v_{enc},\v_{mac}\}~\#~\tv_0 = \cur),\\
  \key{if}~ (\v_{mac} :=: \enc(\v_{enc},\k_M))~ \# ~ \tv_1 = \tv_0 + \tv_{Mac}\\
  \key{then}~ (\key{if}~(\v_{enc} :=: \enc(\v,\k_E)) ~\# ~ \tv_2 = \tv_1 + \tv_{Enc})\\
  \qquad ~\key{then} ~ (+ done ~\#~ \cur = \tv_2)~\key{else}~ (+ error ~\#~ \cur = \tv_2))\\
  \key{else}~(+ error ~\#~ \cur = \tv_1)
\end{array}  
\]
This role creates a fresh value $\v$ and sends it. Then it is expecting a pair of two messages $\v_{mac}$ and $\v_{enc}$, remembering at time variable $\tv_0$ when this message is received. It then checks whether the first component $\v_{mac}$ is of the form $\enc(\v_{enc},\k_M))$, \ie, it is the correct MAC. This operation  takes $\tv_{mac}$ time units. The time variable $\tv_1$ is equal to the time $\tv_0 + \tv_{mac}$, \ie, the time when the message was received plus the MAC check duration. If the MAC is not correct, an $error$ message is sent exactly at time $\tv_1$. Otherwise, if the first component, $\v_{MAC}$, is as expected, the role checks whether the second component, $\v_{enc}$, is an encryption of the form $\enc(\v,\k_E))$, which takes (a longer) time $\tv_{enc}$. If so it sends the $done$ message, otherwise the $error$ message, both at time $\tv_2$ which is $\tv_1 + \tv_{enc}$.
\end{example}

\begin{example}[Red Pill Example]
  We abstract the part of sending the baseline message, \eg, the messages that establish the connection to the server, and the part that sends the differential messages. We assume that it takes \key{dBase} to complete the exchange of the baseline messages.
\[
  \begin{array}{l}
(-(\key{baseline\_req})~ \#~ \tv_0 = \cur),\\
(+(\key{baseline\_done})~ \#~ \cur = \tv_0 + \key{dBase}),\\
(-(\key{diff\_req})~ \#~ \tv_1 = \cur )\\
(+ (\key{diff\_done})~ \#~ \cur = \tv_1 + \key{dAppl})
  \end{array}
\]
Then the part of the protocol that depends on the application starts. We abstract this part using the messages \key{diff\_req} and \key{diff\_done}. If the application is running over a virtual machine, then \key{dAppl} takes \key{dVirtual} time units; otherwise \key{dAppl} takes \key{dReal} time units, where \texttt{dVirtual > dReal}. 

The intruder can distinguish whether an application is running over a virtual machine or not by measuring the time it takes to complete the exchange of \key{diff\_req} and \key{diff\_done} messages. 
\end{example}

\begin{example}[Anonymous Protocol]
  We specify (a simplified version of the) anonymous group protocol proposed by Abadi and Fournet's protocol for private authentication~\cite{abadi04tcs}. Whenever a broadcasted message is received by an agent, it checks whether it has been encrypted with the group key $KB$. If this is the case, then it checks whether the player sending the message with key $\v_G$ is part of the group. If so, then it sends a response encrypted with his private key. Otherwise, he sends a decoy message. 
\[
  \begin{array}{l}
  -(\{\key{hello}), \enc(\{\key{hello},\v_n,\v_G,\},\k_G) \} ~\#~ \tv_0 = \cur\\
  \key{if}~\k_G :=: KB ~\#~ \tv_1 = \tv_0 + \key{dEnc}\\
  \key{then} \\
  \quad \key{if}~\v_G :=: KA ~\#~ \tv_2 = \tv_1 + \key{dCheck}\\
  \quad \key{then}~+(\{\key{ack}, \enc(\key{rsp},\k_B)\}) ~\#~ \cur = \tv_1 + \key{dCreate}\\
  \quad \key{else}~+(\{\key{ack}, \enc(\key{decoy},\k_B)\}) ~\#~ \cur = \tv_1\\
  \key{else}~+(\{\key{ack}, \enc(\key{decoy},\k_B)\}) ~\#~ \cur = \tv_1\\
 %  \begin{verbatim}
 %  (-({t("hello"),     e({t("hello"), nv("A"),v("G")}, kv("M"))} # tt(0) := cur),
 %  eif kv("M") ~ KB # tt(1) := tt(0) + dEnc
 %  ethen
 %    (eif v("G") ~ {KA} # tt(2) := tt(1) + dCheck
 %     ethen +({t("ack"), t("M")} # cur === tt(2) + dCreate)
 %     eelse +({t("ack"), t("M")} # cur === tt(2)) efi)
 % eelse +({t("ack"), t("M")} # cur === tt(1)) efi    
 %  \end{verbatim}
  \end{array}
\]
Notice the use of time constraints to capture that the steps of the protocol take some time, namely \key{dCheck} and \key{dCreate}. 
\end{example}

\subsection{Semantics}

We formalize the semantics of Timed Protocols by extending Strand Spaces and Bundles~\cite{thayer99jcs} to include time constraints and a network topology. 

% \red{Expand this paragraph}

\paragraph{Network Topology} Messages take time to travel between agents, both honest players and intruders. The network model is specified by representing the time a message needs to travel from any agent $a$ to any agent $b$, specified by $\td{a}{b}$ using a function that takes two names and returns a number. Typically, $\td{a}{a} = 0$, that is the time for a message sent from a player to reach himself is 0, but we do not need to enforce this. We also assume the following axiom for all players $a,a_1, \ldots, a_n,a'$ (with $1 \leq n$):
\begin{equation}
  \td{a}{a'} \leq \td{a}{a_1} + \td{a_1}{a_2} + \cdots + \td{a_n}{a'}
\label{eq:geometry}
\end{equation}
That is, it is at least as fast for a message to travel directly from $a$ to $a'$, then to first travel through $a_1,\ldots,a_n$. This is similar to the usual triangle inequality in basic geometry.

A given scenario with some protocol session instances includes the protocol participants (or simply participants), $\Pscr = \{\p_1, \ldots, \p_n\}$ and a set of Timed Intruders $\Iscr = \{\ti_1, \ldots,\ti_m\}$, who may be manipulating messages. The Network Topology is composed by two disjoint functions $\key{td} = \key{td}_\Pscr \uplus \key{td}_\Iscr$ defined as follows:
\[
\td{a}{b} = 
  \left\{ \begin{array}{ll}
    \key{td}_\Pscr(a,b) & \textrm{if $a,b \in \Pscr$}\\
    \key{td}_\Iscr(a,b) & \textrm{otherwise}
  \end{array}\right.
\]
Thus, $\key{td}_\Pscr$ specifies the time messages take to travel among participants, while $\key{td}_\Iscr$ specifies the time messages take to travel between Timed Intruders, between a Timed Intruder and a participant and between a participant and a Timed Intruder. 

\begin{remark}
\label{rem:transmission}
  Here we are assuming that all agents share the same transmission medium for simplicity. It is possible to allow for different communication channel by adding an additional parameter to \key{td}. 
\end{remark}


The following definitions extend Strands and Bundles to include time variables capturing the semantics of Timed Protocols. A Timed Protocol Role is ground if it does not contain variables.

%\paragraph{Timed Strands Spaces and Bundles} 

\begin{definition}
A Timed Strand Space is a set $\Pi$ and a trace mapping $tr : \Pi \lra \Pscr \times \GPL$, where $\Pscr$ is the set of player names $\{\p_1, \ldots, \p_n\}$ and $\GPL$ is the set of Ground Timed Protocol Roles. We denote by $tr(s)_1$ the player name and $tr(s)_2$ the Timed Protocol Role of a strand $s \in \Pi$.
\end{definition}

For the remainder we fix a Timed Strand Space  $[\Pi,tr]$.

\begin{definition} 
\label{def:timed-strands}
The Timed Strand Space Graph, $\Gscr = \tup{\Nscr,\Rightarrow \cup \rightarrow}$, has nodes
$\Nscr$ and edges $\Rightarrow$ and $\rightarrow$ as defined below.
\begin{enumerate}
  \item A node $n$ is a tuple $\tup{\p,s,\bar{i}}@\tv$ with $s \in \Pi$, $\p = tr(s)_1$, $\bar{i}\in \mathcal{PS}(tr(s)_2)$ is a string identifying a command in the Timed Protocol, and $\tv$ is a time variable timestamping the node $n$. The set of nodes is denoted by $\Nscr$;
  \item If $n = \tup{\p,s,\bar{i}}@\tv$, we denote by $term(n)$, the command at position $\bar{i}$ in $tr(s)_2$;
  \item If $n_1 = \tup{\p,s,\bar{i}}@\tv_1$ and $n_2 = \tup{\p,s,\bar{i}.j}@\tv_2$ are in $\Nscr$, then there is an edge $n_1 \Rightarrow n_2$;
  \item For two nodes $\n_1, \n_2 \in \Nscr$, there is an edge $n_1 \rightarrow n_2$ if and only if $term(n_1)$ is of the form $+\m$ or $+\m~\#~\tc_1$ and $term(n_2)$ is of the form $-\m$ or $-\m~\#~\tc_2$;
  \item If a node $n \in \Nscr$,  $term(n) = \new~\c$, then $\c$ originates on $n$, that is, all nodes $n'$ such that $term(n')$ contains $\c$ are such that $n~(\Rightarrow \cup \rightarrow)^* ~n'$, where $(\cdot)^*$ is the reflexive and transitive closure operator.
\end{enumerate}
\end{definition}


\begin{definition}
\label{def:timed-constraint-set} 
Let $\key{td}$ be a Network Topology and let $\Cscr = \tup{\Nscr_\Cscr,\rightarrow_\Cscr \cup \Rightarrow_\Cscr}$ be a subgraph of $\Gscr = \tup{\Nscr,\Rightarrow \cup \rightarrow}$. 
The Timed Constraint Set of $\Cscr$ over $\key{td}$, denoted by $\TC(\Cscr,\key{td})$, is the smallest set of Time Constraints specified as follows:
\begin{enumerate}
  \item If $n = \tup{\p,s,\bar{i}}@\tv \in \Nscr_\Cscr$, such that $term(n)$ is of the form $\pm \m~\#~\tc$ or $\key{if}~{\b~\#~\tc}$, then $\tc' \in \TC(\Cscr,\key{td})$ where $\tc'$ is the Time Constraint obtained by replacing $\cur$ by $\tv$;
  \item If $\tup{\p,s,\bar{i}}@\tv_1 \Rightarrow_\Cscr \tup{\p,s,\bar{i}.j}@\tv_2$, then $\tv_2 \geq \tv_1 \in \TC(\Cscr,\key{td})$;
  \item If $\tup{\p_1,s_1,\bar{i}_1}@\tv_1 \rightarrow_\Cscr \tup{\p_2,s_2,\bar{i}_2}@\tv_2$, then $\tv_2 \geq \tv_1 + \td{\p_1}{\p_2} \in \TC(\Cscr,\key{td})$.
\end{enumerate}
\end{definition}


Intuitively, the $\Rightarrow$ specifies the sequence of actions carried out 
by a protocol session participant, while the $\rightarrow$ specifies the interactions
between protocol sesssion participants. However, not all timed strand space graph will 
correspond to possible executions. Thus, we introduce 
Timed Bundle which is a subset of the Timed Strand space graph, playing a similar role 
of Bundles for Strand Spaces.

\begin{definition} Let $\key{td}$ be a Network Topology. Let $\rightarrow_\Cscr \subseteq \rightarrow$ and $\Rightarrow_\Cscr \subseteq \Rightarrow$ and suppose $\Cscr = \tup{\Nscr_\Cscr,\rightarrow_\Cscr \cup \Rightarrow_\Cscr}$ is a sub-graph of $\tup{\Nscr,\Rightarrow \cup \rightarrow}$. $\Cscr$ is a Timed Bundle over $\key{td}$ if:
\begin{enumerate}
  \item $\Cscr$ is finite and acyclic;
  \item $n_2 \in \Nscr_\Cscr$ is Message Input or a Timed Message Input, then there is a unique $n_1 \in \Nscr_\Cscr$ such that $n_1 \rightarrow_\Cscr n_2$;
  \item  $n_2 \in \Nscr_\Cscr$ and $n_1 \Rightarrow n_2$, then $n_1 \in \Nscr_\Cscr$, and $n_1 \Rightarrow_\Cscr n_2$;
  \item $n = \tup{\p,s,\bar{i}}$ is a node such that $term(n)$ is of the form $\key{if}~{\b}$ or $\key{if}~{\b~\#~\tc}$ and $\b$ is evaluated to true, then $n \Rightarrow_\Cscr \tup{\p,s,\bar{i}.1}$ and  $n \nRightarrow_\Cscr \tup{\p,s,\bar{i}.2}$; otherwise  $n \Rightarrow_\Cscr \tup{\p,s,\bar{i}.2}$ and $n \nRightarrow_\Cscr \tup{\p,s,\bar{i}.1}$;
  \item the Timed Constraint Set of $\Cscr$ over $\key{td}$ is satisfiable, \ie, there is a substitution $\sigma$, called model of $\TC(\Cscr,\key{td})$, replacing all time variables in $\TC(\Cscr,\key{td})$ by Real numbers so that all inequalities in $\TC(\Cscr,\key{td})$ are true.
\end{enumerate}
\end{definition}

\subsection{Timed Intruder Model}

The Timed Intruder Model is similar to the usual Dolev-Yao Intruder Model in the sense that it can compose, decompose, encrypt and decrypt messages provided it has the right keys. However, unlike the Dolev-Yao intruder, a Timed Intruder is constrained by the physical properties of the systems, namely, an intruder is not able to learn any message instantaneously, instead, must wait until the message arrives.

A Timed Intruder Set is a set of intruder names $\Iscr = \{\ti_1,\ldots,\ti_n\}$ a set of initially known keys $K_P$, which contain all  public keys, all private keys of all the intruders, all symmetric keys initially shared between intruders and honest players, and may contain ``lost keys'' that an intruder learned previously by, for instance, succeeding in some cryptoanalysis. Recall that  Timed Intruders are situated at locations specified by the Network Topology. For instance, $\td{\p_1}{\ti_1} = \key{td}_\Iscr({\p_1},{\ti_1}) = 4$ denotes that the timed needed for a message to travel from  participant $\p_1$ to intruder $\ti_1$ is $4$.

\begin{definition}
\label{def:ind-strands}
  An intruder trace is one of the following, where $\ti$ is a Timed Intruder Name, $\tv,\tv_1,\tv_2,\tv_3$ are time variables, and $\m,\m_1,\ldots, \m_n,\m_1',\ldots,\m_p'$ are messages:
  \begin{itemize}
    \item \textrm{Text Message:} $\tup{\ti,+ \t}@\tv$, where $\t$ is a text constant;
    \item Flushing: $\tup{\ti,-\m}@\tv$;
    \item Forward: $\tup{\ti, -\m, +\m}@(\tv_1,\tv_2)$ denoting the strand $\tup{\ti,-\m}@\tv_1 \Rightarrow \tup{\ti,+\m}@\tv_2$;
        % $\tup{\ti, -\m, +\m, +\m}@\tv$, where $\m$ is a message;
    \item Concatenation: \\ $\tup{\ti,-\{\m_1,\ldots,\m_n\}, -\{\m_1',\ldots,\m_p'\},\\ + \{\m_1,\ldots,\m_n,\m_1',\ldots,\m_p'\}}@(\tv_1,\tv_2,\tv_3)$ denoting the strand

    % \vspace{-3mm}
    \begin{small}
    \(
      \begin{array}{l}
     \tup{\ti,-\{\m_1,\ldots,\m_n\}}@\tv_1 \Rightarrow\\  \tup{\ti,-\{\m_1',\ldots,\m_p'\}}@\tv_2 \Rightarrow\\ \tup{\ti,+ \{\m_1,\ldots,\m_n,\m_1',\ldots,\m_p'\}}@\tv_3
       \end{array}
    \)      
    \end{small}
    \item Decomposing: $\tup{\ti,-\{\m_1,\ldots,\m_n\}, +\{\m_1,\ldots,\m_i\},\\+\{\m_{i+1},\ldots,\m_n\} }@(\tv_1,\tv_2,\tv_3)$ denoting the strand

% \vspace{-3mm}
    \begin{small}
     \(
      \begin{array}{l}
     \tup{\ti,-\{\m_1,\ldots,\m_i,\m_{i+1},\ldots,\m_n\}}@\tv_1 \Rightarrow\\ 
\tup{\ti,+\{\m_1,\ldots,\m_i\}}@\tv_2 \Rightarrow\\ \tup{\ti,+ \{\m_{i+1},\ldots,\m_n\}}@\tv_3
       \end{array}       
     \)      
    \end{small}
    \item Key: $\tup{\ti,+\k}@\tv$ if $\k \in K_P$;
    \item Encryption: $\tup{\ti,-\k,-\m,+\enc(\m,\k)}@(\tv_1,\tv_2,\tv_3)$ denoting the strand

    \(
    \begin{array}{c}
    \tup{\ti,-\k}@\tv_1 \Rightarrow  \tup{\ti,-\m}@\tv_2 \Rightarrow  \tup{\ti,+\enc(\m,\k)}@\tv_3      
    \end{array}
    \)
    \item Decryption: $\tup{\ti,-\k^{-1},-\enc(\m,\k),+\m}@(\tv_1,\tv_2,\tv_3)$.

    \(
    \begin{array}{c}
    \tup{\ti,-\k^{-1}}@\tv_1 \Rightarrow  \tup{\ti,-\enc(\m,\k)}@\tv_2 \Rightarrow  \tup{\ti,+\m}@\tv_3      
    \end{array}
    \)
  \end{itemize}
\end{definition}

As with the the usual Dolev-Yao intruder model as, e.g., in \cite{thayer99jcs}, the Timed Intruder can send text messages and known keys, receive a message, replay a message, concatenate and decompose messages, and finally encrypt and decrypt messages. There are, however, two differences with respect to the usual Dolev-Yao intruder model as defined in \cite{thayer99jcs}. Each node of the trace is associated with an intruder name $\ti$ and a time variable $\tv$. These are necessary for extracting the Time Constraints of a Strand Graph (as described in Definition~\ref{def:timed-constraint-set}), specifying the physical restrictions of the Timed Intruder.

As the time when timed intruders receive and manipulate messages cannot be measured by the protocol participants, they do not have control over the time variables of timed intruder strands. The following assumption captures this intuition:

\paragraph{Time Variable Disjointness Assumption} For any Bundle $\Bscr$, the set of time variables appearing in protocol participant strands in $\Bscr$ is disjoint from the set of time variables appearing in timed intruder strands in $\Bscr$.

\begin{figure*}[t]
\begin{center}
  \includegraphics[width=0.8\textwidth]{figs/strand-distance-bounding-mafia.pdf}
\end{center}  
\caption{Bundle for the mafia attack described in Example~\ref{ex:mafia-attack}.}
\label{fig:strand-mafia}
\end{figure*}


\begin{example} 
\label{ex:mafia-attack}
Let us return to the distance bounding protocol described in 
Example~\ref{ex:distance-bounding}. The following is an attack, where two colluding intruders $\ti_1$, who is close to $\p_1$, and $\ti_2$, who is close to $\p_2$, collude by sharing a fast channel to fool $\p_1$ into thinking that $\p_2$ is closer than he actually is.

The intruders $\ti_1$ and $\ti_2$ simply forward messages between each other and the players $\p_1$ and $\p_2$. However, this is a Bundle only if the following Time Constraint Set is satisfiable:
\[
\left\{
\begin{array}{c}
  \tv_2 \geq \tv_1, \tv = \tv_2, \tv_6 \geq \tv_2 + \td{\p_1}{\ti_1}, \tv_7 \geq \tv_6,\\
   \tv_8 \geq \tv_7 + \td{\ti_1}{\ti_2}, \tv_9 \geq \tv_8,
  \tv_4 \geq \tv_9 + \td{\ti_1}{\p_2},\\ \tv_5 \geq \tv_4,
   \tv_{10} \geq \tv_5 + \td{\p_2}{\ti_1}, \tv_{11} \geq \tv_{10},\\ \tv_{12} \geq \tv_{11} + \td{\ti_2}{\ti_1}, \tv_{13} \geq \tv_{12}, \tv_3 \geq \tv_{13} + \td{\ti_1}{\p_1},\\ \tv_3 \leq \tv_2 + 4
\end{array}
\right\}
\]
This set of constraints represents a set of concrete executions, where the Timed Intruders $\ti_1$ and $\ti_2$ collude. There is a concrete execution only if the set of Time Constraints is satisfiable, \ie, it has a \emph{model}, which depends on the Network Topology, that is, on the function $\key{td}$. 
\end{example}

\begin{definition}
  A \emph{time model} $M$ of a set of time constraints $\Tscr$ is a mapping from the time variables in $\Tscr$ to non-negative real numbers such that all constraints in $\Tscr$ are satisfied.
\end{definition}

For example, the following model 
\[
M = \{\tv_1 \mapsto 2.0, \tv_2 \mapsto 2.2, \tv_3 \mapsto 1.8 \} 
\]
is a model of the following set of time constraints:
\[
 \Tscr = \{\tv_1 \leq \tv_2, \tv_3 \leq \tv_1 + 1.0, \tv_2 > \tv_3\}.
\]
We write $M \vDash \Tscr$ if $M$ is a model of the constraints $\Tscr$.


\begin{definition}\label{init}
  An initial configuration is a tuple 
\[
  I = \tup{\Hscr, \Iscr, \key{td}}
\]
where  $\Hscr = \{(\p_1,\pl_1), \ldots, (\p_n,\pl_n)\}$ is a set of honest players with their corresponding timed protocols; $\Iscr = \{(\ti_1,\IK_1), \ldots, (\ti_m,\IK_m)\}$ is a set of timed intruders with their corresponding intruder strands, representing initial intruder knowledge; and  \key{td} is a network topology. Moreover, the sematics, $\Sscr(I)$, of an initial configuration is the set of timed bundles of $I$, representing the possible executions of $I$.
\end{definition}



==> stobseq.tex <==
%!TEX root = obseq.tex
\section{Symbolic Timed Observational Equivalence}\label{stobseq}

Intuitively, two systems $s_1$ and $s_2$, modeled by two initial configurations, are equivalent if there is no behavior of $s_1$ that cannot be emulated by $s_2$ and vice-versa. This notion is formalized by using the notion of observational equivalence: 

\begin{definition}
  Two systems, $s_1$ and $s_2$, are observational equivalent, written $s_1 \equiv s_2$ if $s_1 \preceq s_2$ and $s_2 \preceq s_1$, where $s_i \preceq s_j$ if for all contexts $C[\cdot]$, we have that $C[s_i]$ has the same \emph{observations} as $C[s_j]$. 
 \end{definition} 

The notion of observation will vary according to the application domain. For example, the equivalence in programming languages is concerned with a
value produced. Protocol security is also interested in the order in which messages are sent by honest participants. Here, we will also be interested in the time when messages are sent. We will formalize this in Section~\ref{subsec:observations}.


A number of security protocol properties, such as anonimity, unlinkability, and privacy, have been reduced to the problem of observational equivalence~\cite{arapinis10csf}. Thus it is a powerful notion for discovering non-trivial flaws in protocols. 

However, one main problem for automated verification in using the above definition  is the quantification over contexts. There have been, however, many techniques developed that overcome this problem and can be used for proving the equivalence of systems, \eg, logical relations~\cite{gunter,hofmann14popl}, bisimulation~\cite{milner}. 

The problem of quantification of contexts in protocol security verification can be overcome by relying on the following fact~\cite{cervesato02isss}:

\begin{center}
\textbf{Fact:} The Dolev-Yao intruder is the most powerful intruder.   
\end{center}

Thus, it is not necessary for (traditional) protocol security verification to check whether for all contexts the systems evaluate to the same value, but rather check this for a single context implementing the Dolev-Yao intruder. All \emph{observations} obtained by any (symbolic) context can be observed by the Dolev-Yao intruder. 

Unfortunately, the Dolev-Yao intruder is not suitable for cyber-physical protocol security verification because the Dolev-Yao intruder is too strong, being faster than the speed of light. Therefore, one should use instead a weaker timed Dolev-Yao intruder which is not omnipresent, but is placed at some location~\cite{kanovich14fccfcs}. It only may learn a message when it arrives, \ie, a timed intruder needs to wait for the message to travel from the sender to him. Thus, the observed behaviors depends on the context, \ie, number of intruders and their location and therefore, we face again the problem of quantifying over all contexts. 

To solve this problem, we rely on the following result from~\cite{nigam16esorics} which formalizes \emph{timed intruder models} and proves the following fact:
\begin{center}
  \textbf{Fact:} Timed intruders located at \emph{negligible} distance to honest participants (one intruder per participant) is the strongest timed intruder configuration.
\end{center}
That is, any observation resulting from a context where timed intruders are placed differently can also be observed if the timed intruders are placed at negligible distance to the honest participants. 

Therefore, it is enough for protocol verification to consider a single context where timed intruders are placed at neglible distance to honest participants. Formally, this means that for each participant $p$ there is a timed intruder $I_p$ such that:
\[
\begin{array}{l}
  \key{td}_\Iscr(I_p,I_q) = 
  \key{td}_\Iscr(p,I_q) = \key{td}_\Iscr(I_p,q) =  \key{td}(p,q)\\
  \key{td}_\Iscr(p,I_p) =  \key{td}_\Iscr(I_p,p) = 0\\
\end{array}
\]

If we were to assume additional communication channels (see Remark~\ref{rem:transmission}), then we would assume that the intruders always communicate with the channel with the greatest speed.


 % From this point, we assume that each honest participant there is an associated timed intruder placed at the same location. 


\subsection{Observations}
\label{subsec:observations}
Assume that we are given a initial configuration $I$ (definition \ref{init})
We are interested in the set of observations that can be obtained by executing $I$ where the timed intruders are located at negligible distance to honest participants. Intuitively, an observation will be the messages that intruders learn as in usual protocol security verification~\cite{cortier09csf} together with the time when a message was sent. That is, the messages that are sent into the network. 

Formally, an observation has the following format:
\begin{definition}
\label{def:message-observation}
  A \emph{message observation} is a tuple $\tup{msg,snd,rcv,time}$ where $msg$ is the message exchanged, $snd$ is the player that sent the message $msg$, $rcv$ is the player that received the message $msg$, and the $time$ is the time when the message is sent.
\end{definition}

The following definition formalizes the set of observations of a timed bundle by looking only at the $n_1 \to n_2$ edges between honest participants and associated timed intruders. 

Notice that we do not need to keep the time of receipt of messages as from our timed intruder model assumption (see the text just before Section~\ref{subsec:observations}), the intruder is negligibly close 
to the sender and message transmission is instantaneous.

\red{Maybe only look at intruder outputs.}

\begin{definition}
 Let $\Cscr = \tup{\Nscr_\Cscr,\rightarrow_\Cscr \cup \Rightarrow_\Cscr}$ be a timed bundle over a network topology $\key{td}$. The set of observations of $\Cscr$ is a pair composed by the set of message observations, written $\Oscr(\Cscr)$, below and the Timed Constraint Set of $\Cscr$, $\TC(\Cscr,\key{td})$:
\[
\hspace{-4mm}
\left\{ \begin{array}{lcl}
  \tup{\m,\p_S,\p_R,\tv_0} & \mid &  n_1 \to  n_2 \land time(n_1) = \tv_0 \land~ \\
  && player(n_1) = \p \land player(n_2) = \p_R\\ 
  && (term(n_1) = +\m \lor~\\
  && term(n_1) = +\m~\#~\tc)
\end{array}
\right\}
\] 
\end{definition}

Consider Example~\ref{ex:mafia-attack} and the timed bundle depicted in Figure~\ref{fig:strand-mafia}. The observations of this timed bundle is the pair composed by the timed constraint shown in Example~\ref{ex:mafia-attack} and the following set of message observations:
\[
\left\{ \begin{array}{c}
  \tup{\c,\p_1,I,\tv_2}, \tup{\c,I,\p_2,\tv_9},
  \tup{\c,\p_2,I,\tv_{5}}, \tup{\c,I,\p_1,\tv_{13}}
\end{array}\right\}
\]

\subsection{Timed Equivalence}

In order to define timed equivalence, we need to describe when two messages seem identical to an external intruder. In symbolic verification using Dolev-Yao like intruders, one assumes that the intruder cannot distinguish two encrypted messages if the intruders do not possess the corresponding encryption keys. The following definitions makes this precise.


\red{Add that nonces are also indistinguishable.}
\begin{definition}
  Two messages $\m_1$ and $\m_2$ are similar, written $\m_1 \sim \m_2$ if and only if:
  \begin{itemize}
    \item $\m_1$ and $\m_2$ are both constants and $\m_1 = \m_2 = \c$;
    \item $\m_1 = \enc(\m_1',\k_1)$ and $\m_2 = \enc(\m_2',\k_2)$;
    \item $\m_1 = \{\m_1',\ldots,\m_n'\}$ and 
    $\m_2 = \{\m_1'',\ldots,\m_n''\}$ and for all $1 \leq i \leq n$, $\m_i' \sim \m_i''$.
  \end{itemize}
\end{definition}

Two messages that are similar may be distinguishable by an intruder. It will depend on the overall knowledge acquired by the intruder in the bundle, namely the keys he has learned. For example, consider the following two timed bundles, $\Bscr_1$ and $\Bscr_2$, where the first two messages are permuted. We omit  the time variables and the intruder strands.
\[
\begin{array}{l}
 \Bscr_1 = \tup{\p_1,+\enc(\c_1,\k)} \Rightarrow \tup{\p_1,+\enc(\c_2,\k)} \Rightarrow \tup{\p_1,+\k};\\
  \Bscr_2 = \tup{\p_1,+\enc(\c_2,\k)} \Rightarrow \tup{\p_1,+\enc(\c_1,\k)} \Rightarrow \tup{\p_1,+\k};  
\end{array}
\]
Assuming the intruder does not possess the key $\k$, \ie, $\k \notin K_P$, the intruder cannot distinguish the messages $\enc(\c_1,k)$ and $\enc(\c_2,k)$ when these are sent. However, once he learns the corresponding key $\k$ due to the third message, he can distinguish $\enc(\c_1,k_1)$ and $\enc(\c_2,k_2)$ and therefore distinguish these timed bundles. 

Therefore, to check whether two messages are distinguishable depends on the intruder knowledge. This can be formalized by using the notion of derivable messages as follows:

\begin{definition}
  Let $\IK$ be a set of strands available to the intruders which includes the strands in Definition~\ref{def:ind-strands} and any initial knowledge. Let $\ti$ be any intruder.
   Let $\Kscr(\IK)$ be the set of keys that the intruder can construct:
    \[
      \hspace{-3mm}
    \Kscr(\IK) =
 \left\{\begin{array}{lcl}
  \k & \mid & \textrm{It is possible to construct a bundle } \\
  && \textrm{outputting $\k$ using the strands in $\IK$ }
\end{array}\right \}
  \]
  We define the set of derivable terms, $\DC(\m,\IK)$, for a given message $\m$ as $\DC(\m,\IK) =$
  \[
  \hspace{-5mm}
\left\{\begin{array}{lcl}
  \m' & \mid & \textrm{It is possible to construct a bundle } \\
  && \textrm{outputting $\m'$ using the strands Decomposing,}\\ 
  && \textrm{Decryption, $\tup{\ti,\k}@\tv_1$ and $\tup{\ti,-\m,+\m}@\{\tv_2,\tv_3\}$}\\
  && \textrm{for fresh symbols $\tv_1,\tv_2,\tv_3$ and $\k \in \Kscr(\IK)$.}
\end{array}\right \}
  \]
  Moreover, we define $\DC(\m_1,\IK_1) \sim \DC(\m_2,\IK_2)$ if for all $\m_1' \in \DC(\m_1,\IK_1)$ there is a $\m_2' \in \DC(\m_1,\IK_1)$ such that $\m_1' \sim \m_2'$ and vice versa.
\end{definition}

For example, in the bundles $\Bscr_1$ and $\Bscr_2$ above, for the intruder strand space $\IK$, the intruders have the following keys where $K_P$ are the initially known keys and $\k \notin K_P$:
\[
  \Kscr(\IK) = \{\k\} \cup K_P
\]
With this set of keys, the intruders can distinguish the messages $\enc(\c_1,\k)$ and $\enc(\c_2,\k)$. This is formally captured by using the derivable sets $\DC$:
\[
  \DC(\enc(\c_1,\k),\IK) \nsim \DC(\enc(\c_2,\k),\IK)
\]
This is because in the set to the left the intruder can output $\c_1$, while this is not the case in the set to the right.

% The definition of $\DC$ leads to possibly infinite sets of derivable terms. In the next section, we explain how we deal with this problem using symbolic terms and constraint systems. 

The following definitions formalize timed observational equivalence. Intuitively, it says that a timed bundle $\Cscr_1$ can be approximated by another timed bundle $\Cscr_2$ if all observations of messages and their sending times can be matched by observations in  $\Cscr_2$.

\begin{definition}
\label{def:approx}
  Let $\Cscr_1$ and $\Cscr_2$ be two timed bundles over the same network \key{td}. Let $\IK_1$ and $\IK_2$ be the intruder strands in, respectively, $\Cscr_1$ and $\Cscr_2$. We say that $\Cscr_1$ is approximated by $\Cscr_2$, written $\Cscr_1 \preceq \Cscr_2$, if and only if
\[
\hspace{-5mm}
\begin{array}{l}
% |\Oscr(\Cscr_1)| = |\Oscr(\Cscr_2)| \land~ \\
  \forall M_1. (M_1 \vDash \TC(\Cscr_1,\key{td})\Rightarrow \exists M_2. (M_2 \vDash \TC(\Cscr_2,\key{td})\Rightarrow\\
  ~\exists B : \Oscr(\Cscr_1) \to \Oscr(\Cscr_2). (\textrm{$B$ is a bijection}\Rightarrow~\\ 
  \quad \forall \tup{\m_1,\p_S,\p_R,\tv_1} \in \Oscr(\Cscr_1).\\
  \qquad B(\tup{\m_1,\p_S,\p_R,\tv_1}) = \tup{\m_2,\p_S,\p_R,\tv_2}\Rightarrow~\\
  ~\qquad \DC(\m_1,\IK_1) \sim \DC(\m_2,\IK_2) \land M_1[\tv_1] = M_2[\tv_2]))).
\end{array}
\]
% For all time models $M_1$ of $\TC(\Cscr_1,\key{td})$, there exists a time model of $\TC(\Cscr_2,\key{td})$ such that for all for all message observations $\tup{\m_1,\p_S,\p_R,\tv_1}$ in $\Cscr_1$ there is a message observation $\tup{\m_2,\p_S,\p_R,\tv_2}$ in $\Cscr_2$ such that:
% \begin{itemize}
  % \item \textbf{(Same term observable)} $\DC(\m_1,\IK_1) = \DC(\m_2,\IK_2)$;
  % \item \textbf{(Same observed time)} $M[\tv_1] = M[\tv_2]$.
% \end{itemize}
\end{definition}

\begin{definition}[Timed Bundles Equivalence]
Let $\Cscr_1$ and $\Cscr_2$ be two timed bundles over the same network \key{td}. We say that $\Cscr_1$ and $\Cscr_2$ are observational equivalent, written $\Cscr_1 \equiv \Cscr_2$ if and only if $\Cscr_1 \preceq \Cscr_2$ and $\Cscr_2 \preceq \Cscr_1$.  
\end{definition}

The definition of approximation (Definition~\ref{def:approx}) contains a quantification over all possible models $M_1$ of $\TC(\Cscr_1,\key{td})$. This will need to be overcome in order to automate the verification of timed observational equivalence. We explain in the next section how we handle this using SMT solvers. 

Moreover, notice the need for a bijection, $B$, between $\Oscr(\Cscr_1)$ and  $\Oscr(\Cscr_2)$. Such bijection should exist, otherwise the following timed bundles would be equivalent:
\[
\begin{array}{l}
  \Bscr_3 = \tup{\p_1, +\c_1}  \\
  \Bscr_4 = \tup{\p_1, +\c_1} \Rightarrow \tup{\p_1, +\c_1}
\end{array}
\]
However, they can be distinguished as in $\Bscr_3$ intruders observe only one message, while in $\Bscr_4$, they see two messages. 

\begin{figure*}[ht]
  \includegraphics[width=0.50\textwidth]{figs/passport.pdf}
  \includegraphics[width=0.50\textwidth]{figs/passport2.pdf}
  \caption{Timed bundles of the passport example (Example~\ref{ex:passport}) when the intruder is meeting a passport previously seen and a passport not previously seen.}
  \label{fig:passport-bundles}
\end{figure*}

We illustrate the definition of timed observational equivalence with the timed bundles shown in Figure~\ref{fig:passport-bundles} for the passport protocol described in Example~\ref{ex:passport}. Assume that the intruder has obtained the messages $\m_{enc}^{old}$ and $\m_{mac}^{old}$ from a previous interaction with a given passport. Figure~\ref{fig:passport-bundles} depicts the timed bundles, $\Cscr_1$ to the left, when the intruder is interacting with the same passport and the timed bundle, $\Cscr_2$ to the right, when the intruder is interacting with a different passport not previously seen. 

The set of observation messages in $\Cscr_1$ and $\Cscr_2$ are the same (modulo time variable renaming). They differ, however, on their timed constraints $\TC(\Cscr_1,\key{td})$ and $\TC(\Cscr_2,\key{td})$. The former contains the constraints:
\[
  \{\tv_{17} = \tv'', \tv'' = \tv' + \tv_{enc}, \tv' = \tv + \tv_{mac}, \tv == \tv_{14}\}
\]
where $\tv_{17}$ is the time when the message $\key{error}$ is sent. On the other hand, $\TC(\Cscr_2,\key{td})$ contains the following set of timed constraints:
\[
  \{\tv_{16} = \tv', \tv' = \tv + \tv_{mac}, \tv == \tv_{14}\}
\]
where $\tv_{16}$ is the time when the message $\key{error}$ is sent. 

Assuming $\tv_{enc}, \tv_{mac}$ fixed, say 1.0, we have that $\Cscr_1$ and $\Cscr_2$ are not observational equivalent. Consider the a model, $M_2$ of $\TC(\Cscr_2,\key{td})$ containing the assignments:
\[\left\{ 
\begin{array}{c}
  \tv_{13} \mapsto 1.0, \tv_{14} \mapsto 1.0, \tv \mapsto 0, 
    \tv' \mapsto 2.0, \tv_{16} \mapsto 2.0  
\end{array}\right\}
\]
This means that the message $\tup{\m_{mac}^{old},\m_{enc}^{old}}$ is sent at time 1.0 and the message $\key{error}$ is sent at time $\tv_{16} = 2.0$. 

It is not possible to find a model $M_1$ of $\TC(\Cscr_1,\key{td})$ where $\tup{\m_{mac}^{old},\m_{enc}^{old}}$ is sent at time 1.0, \ie, $\tv_{14} \mapsto 1.0$ and $\key{error}$ is sent at time $\tv_{17} \mapsto 2.0$ as the constraints entail that
$\tv_{17} = \tv_{enc} + \tv_{mac} + \tv_{14}$.

% \red{How about definitions with different networks?}

\begin{definition}
  Let $I_1$ and $I_2$ be two initial configurations over the same network \key{td}. $I_1$ is timed equivalent to $I_2$ if for all timed bundles $\Cscr_1$ of $\Sscr(I_1)$ there is a timed bundle $\Cscr_2$ of $\Sscr(I_2)$ such that $\Cscr_1 \equiv \Cscr_2$ and conversely.
\end{definition}

==> timed.tex <==
%!TEX root = obseq.tex

\subsection{Timed Observational Equivalence}

We extend the definition of observables to include  (multiple) timed intruders and time constraints:
\begin{definition}
  Let $\tau = \Cscr_1 \stackrel{l_1}{\lra} \Cscr_2 \stackrel{l_2}{\lra} \cdots \stackrel{l_{n-1}}{\lra} \Cscr_n = \tup{\Pscr_n,\DY_n,\DC_n,\EQ_n,\TC_n}@\tG_n$ be a timed trace. Its observable is the tuple $\tup{\tv_I,\Lscr_\tau,\IK,\DC_n,\EQ_n,\TC_n}$, where $\tv_I$ is the global time at configuration $\Cscr_1$, $\Lscr_\tau$ is the sequence of labels in $\tau$ and 
  \[
    \IK = \bigcup_{[i, \IK_i, \buf_i] \in \DY_n} \IK_i
  \]
  is the knowledge accumulated by all intruders.
\end{definition}

Notice that at the end we collect the knowledge accumulated by all intruders. This is because given time, they would have enough time to share all data gathered. We now extend the notion of observable equivalence. For this, assume two sets of observables $\Oscr$ and $\Oscr'$ with disjoint sets of symbols, disjoint sets of nonce names and disjoint sets of time variable names. 

\begin{definition}
\label{def:timed-obs}
  Let $\Oscr = \tup{\tv_I,\Lscr, \IK, \DC,\EQ,\TC}$ and $\Oscr' = \tup{\tv_I',\Lscr', \IK', \DC',\EQ',\TC'}$ be two timed observables, such that $\Lscr = \{(\pm_1 \ms_1 @ \tG_1) \ldots (\pm_p \ms_p @ \tG_p)\}$ and $\Lscr' =\{(\pm_1' \ms_1' @ \tG_1') \ldots (\pm_n' \ms_n' @ \tG_n')\}$. Assume $\widetilde{\tv}$ and $\widetilde{\tv'}$ are the set of time variables in $\TC$ and $\TC'$, respectively. The observation $\Oscr$ is equivalent to $\Oscr'$, written $\Oscr \sim \Oscr'$ if the following conditions are all true:
  \begin{enumerate}
    \item 
    \label{defitem:timed-obs1}
    The branching observables  $\tup{\Lscr,\IK,\DC,\EQ},\tup{\Lscr',\IK',\DC',\EQ'}$ are equivalent where they are obtained from $\Oscr,\Oscr'$ respectively, by eliding all time variables. Thus $p = n = N$
    \item The following formula is a tautology:
    \[
      \forall \widetilde{\tv}. \left[\TC \Rightarrow \exists \widetilde{\tv'}. \left[\TC' \land 
      \tG_1 = \tG_1' \land \cdots \land \tG_N = \tG_N' \right]\right]
    \]
    specifying that for any time $\tG_1, \ldots, \tG_N$ satisfying $\TC$ when the messages $\ms_1, \ldots, \ms_N$ were observed in $\Oscr$, we can find $\tG_1', \ldots, \tG_N'$ satisfying $\TC'$, that makes the time of observation equal.
    \label{defitem:timed-obs2}
  \end{enumerate}
\end{definition}

For Condition~\ref{def:timed-obs}.\ref{defitem:timed-obs1}, we simply use the function $\termEqApprox$ introduced in the previous Section. For Condition~\ref{def:timed-obs}.\ref{defitem:timed-obs2}, we reduce it to a formula for which existing solvers can be used~\cite{duterte15smt}, namely formulas of the form $\exists \forall$:
    \[
    \begin{array}{l}
      \forall \widetilde{\tv}. \left[\TC \Rightarrow \exists \widetilde{\tv'}. \left[\TC' \land 
      \tG_1 = \tG_1' \land \cdots \land \tG_N = \tG_N' \right]\right] \textrm{is a tautology}\\[2pt]
      \Leftrightarrow
      \neg \forall \widetilde{\tv}. \left[\TC \Rightarrow \exists \widetilde{\tv'}. \left[\TC' \land 
      \tG_1 = \tG_1' \land \cdots \land \tG_N = \tG_N' \right]\right] \textrm{is unsat}
      \\[2pt]
      \Leftrightarrow \exists \widetilde{\tv}. \left[\TC \land \forall \widetilde{\tv'}. \left[ \TC' \Rightarrow \neg \left[ 
      \tG_1 = \tG_1' \land \cdots \land \tG_N = \tG_N' \right] \right]\right] \textrm{is unsat}\\
    \end{array}
    \]
In our implementation, we use the SMT solver Yices for solving this formula (which is decidable as shown by Tarski), where all time variables have type Reals. 


\begin{theorem}
Determining whether two timed observables are equivalent is decidable.
\end{theorem}



